PUMA: Deep Metric Imitation Learning for Stable Motion Primitives

Imitation Learning (IL) is a powerful technique for intuitive robotic programming. However, ensuring the reliability of learned behaviors remains a challenge. In the context of reaching motions, a robot should consistently reach its goal, regardless of its initial conditions. To meet this requirement, IL methods often employ specialized function approximators that guarantee this property by construction. Although effective, these approaches come with a set of limitations: 1) they are unable to fully exploit the capabilities of modern Deep Neural Network (DNN) architectures, 2) some are restricted in the family of motions they can model, resulting in suboptimal IL capabilities, and 3) they require explicit extensions to account for the geometry of motions that consider orientations. To address these challenges, we introduce a novel stability loss function, drawing inspiration from the triplet loss used in the deep metric learning literature. This loss does not constrain the DNN's architecture and enables learning policies that yield accurate results. Furthermore, it is not restricted to a specific state space geometry; therefore, it can easily incorporate the geometry of the robot's state space. We provide a proof of the stability properties induced by this loss and empirically validate our method in various settings. These settings include Euclidean and non-Euclidean state spaces, as well as first-order and second-order motions, both in simulation and with real robots. More details about the experimental results can be found in: https://youtu.be/ZWKLGntCI6w.

==> sections/sphere_pose.tex <==
\subsubsection{n-spheres as poses}
The question now arises whether it is possible to represent both positions and orientations together on an n-sphere. To clarify, in $n=3$, if we represent the position in $\mathbb{R}^{3}$ and the orientation in $\mathcal{S}^{3}$ (unit quaternion), can we find a diffeomorphism of the form $\mathbb{R}^{3} \times \mathcal{S}^{3} \to {\mathcal{S}^{6}}'$? A positive answer would indicate that PUMA can use n-spheres in the latent space to represent poses mapped from $\mathbb{R}^{3} \times \mathcal{S}^{3}$ and enforce their stability.

The manifold $\mathbb{R}^{3} \times \mathcal{S}^{3}$ can be conceptualized as points residing on a 3-sphere, each paired with a corresponding hyperplane. Therefore, the entire manifold integrates the 3-sphere with its associated tangent spaces. Figure \ref{fig:dual} illustrates this concept in two dimensions, i.e., $\mathbb{R}^{1} \times \mathcal{S}^{1}$. Interestingly, this construction resembles the manifold of \emph{unit dual quaternions} \cite{clifford1871preliminary, selig2005geometric}. These dual quaternions are utilized for pose representation, offering a unified, compact, and singularity-free space. The resemblance suggests an opportunity for deeper exploration of these concepts in future work, potentially involving unit dual quaternions.

Building on this understanding, we hypothesize that it is possible to find a diffeomorphism between $\mathbb{R}^{3} \times \mathcal{S}^{3}$ and ${\mathcal{S}^{6}}'$, as represented in Fig. \ref{fig:dual}. In this simplified illustration, the figure shows how performing a $\pi/2$ rotation of each associated hyperplane (in this case, lines) with respect to the normal of the circle at each point can create a spherical representation of the pose. The same idea can be extrapolated to higher-dimensional manifolds, such as $\mathbb{R}^{3} \times \mathcal{S}^{3}$.

This hypothesis carries a significant implication. It suggests that if PUMA uses a metric in $\ell_{\text{stable}}$ that enables the learning of a spherical manifold in $\mathcal{L}$ (e.g., Euclidean or great circle distance), it could enforce stability in the motion of poses. We evaluate this idea in Section \ref{sec:real_world}.

==> sections/sphere_pose_old.tex <==
\subsubsection{n-spheres as poses}
The question now arises whether it is possible to represent both positions and orientations together on an n-sphere. To clarify, in 3 dimensions, if we represent the position in $\mathbb{R}^{3}$ and the orientation in $\mathcal{S}^{3}$ (unit quaternion), can we find a diffeomorphism of the form $\mathcal{S}^{3} \ltimes \mathbb{R}^{3} \to {\mathcal{S}^{6}}'$\footnote{Note the semidirect product $\ltimes$ is employed as quaternion algebra is non-commutative.}? A positive answer would indicate that PUMA can use n-spheres in the latent space to represent poses.

\emph{Dual quaternions} \cite{clifford1871preliminary} are helpful in this, given that a specific subset, the \emph{unit dual quaternions}, belongs to $\mathcal{S}^{3} \ltimes \mathbb{R}^{3}$\footnote{This space is commonly expressed in the form $\text{Spin}(3) \ltimes \mathbb{R}^{3}$ \cite{selig2005geometric}; however, $\text{Spin}(3)$ is homeomorphic to $S^{3}$ \cite{lawson1989spin}.}. A dual quaternion $\sigma$ is defined as
\begin{equation}
    \sigma = p + \epsilon q
\end{equation}
where $p$ and $q$ are quaternions and $\epsilon$ is the \emph{dual unit} with $\epsilon^{2}=0$ and $\epsilon \neq 0$. Here, $p$ represents the orientation and $q$ contains the information on the position of a pose. While the dual quaternion exists in an 8-dimensional space due to its two quaternion components, its structure allows for the definition of unit dual quaternions that satisfy the following constraints:
\begin{align}
    |p| = 1, \label{eq:1}\\
    p \cdot q = 0. \label{eq:2}
\end{align}
Consequently, the dimensionality reduces, and unit dual quaternions become 6-dimensional manifolds. Notably, constraint \eqref{eq:1} ensures that the orientation quaternion $q$ maintains a unit norm, thereby preserving the properties inherent to unit quaternions. On the other hand, constraint \eqref{eq:2} dictates that both quaternions must be orthogonal. This mathematical structure enables us to conceptualize unit dual quaternions as points residing on the 3-sphere, representative of orientations, paired with a corresponding hyperplane representing the position \cite{jia2013dual}. Therefore, the complete manifold integrates the 3-sphere with all its corresponding tangent spaces. A 2-dimensional visualization is depicted in Fig. \ref{fig:dual}.

Building on this understanding, it is intriguing to consider the potential applicability of ${\mathcal{S}^{6}}'$ for the representation of unit dual quaternions. This idea is founded on the possibility of establishing a diffeomorphism between these entities, a concept visually represented in Fig. \ref{fig:dual}. This figure presents a 2-dimensional representation of unit dual quaternions. Then, by performing a $\pi/2$ rotation of each associated hyperplane (in this case, lines) perpendicular to the circle for every orientation, a mapping can be made to a subset of a sphere. This suggests that, since unit dual quaternions can be represented within $\mathbb{R}^{3} \times \mathcal{S}^{3}$, a bijection may be drawn between this manifold and ${\mathcal{S}^{6}}'$.

This statement carries a substantial implication. Specifically, it suggests that provided PUMA utilizes a metric in $\ell_{\text{stable}}$ that enables the learning of a spherical manifold in $\mathcal{L}$ (for instance, Euclidean or great circle distance), it would be possible to enforce stability in the motion of poses.
